The Random-Cluster Model

The class of random-cluster models is a unification of a variety of stochastic processes of significance for probability and statistical physics, including percolation, Ising, and Potts models; in addition, their study has impact on the theory of certain random combinatorial structures, and of electrical networks. Much (but not all) of the physical theory of Ising/Potts models is best implemented in the context of the random-cluster representation. This systematic summary of random-cluster models includes accounts of the fundamental methods and inequalities, the uniqueness and specification of infinite-volume measures, the existence and nature of the phase transition, and the structure of the subcritical and supercritical phases. The theory for two-dimensional lattices is better developed than for three and more dimensions. There is a rich collection of open problems, including some of substantial significance for the general area of disordered systems, and these are highlighted when encountered. Amongst the major open questions, there is the problem of ascertaining the exact nature of the phase transition for general values of the cluster-weighting factor q, and the problem of proving that the critical random-cluster model in two dimensions, with 1\le q\le 4, converges when re-scaled to a stochastic L\"owner evolution. Overall the emphasis is upon the random-cluster model for its own sake, rather than upon its applications to Ising and Potts systems.

==> emslab.tex <==
\ifx\labelsloaded\relax\endinput\else\let\labelsloaded\relax\fi
\catcode`\@=11 % Letter
%
\newwrite\@auxout
\newif\if@fwdref \@fwdreffalse
 
%      **************************
%      *       COUNTERS         *
%      **************************
%
\newcount\Thm@nro \Thm@nro=0
\newcount\Sec@nro \Sec@nro=0
\newcount\SubSec@nro \SubSec@nro=0
\newcount\Item@nro \Item@nro=0
%
\def\theThm{\the\Thm@nro}
\def\theSec{\the\Sec@nro}
\def\theSubSec{\the\SubSec@nro}
\def\theItem{\the\Item@nro}
%
%
\def\stepbyone#1{\global\expandafter
  \advance\csname#1@nro\endcsname by1\relax}
\def\stepcounter#1#2{\global\expandafter
  \advance\csname#1@nro\endcsname by #2\relax}
\def\setcounter#1#2{\global\expandafter\csname#1@nro\endcsname =#2\relax}
 
\def\Thm@#1{\xdef\@currentlabel{#1\LeftTagForm%
    \ifnum\Thm@nro=0
    \else\ifnum\Sec@nro=0 \theThm
	 \else
    		\ifnum\SubSec@nro=0 \theSec.\theThm
                \else\theSec.\theSubSec.\theThm
        	\fi
	 \fi
    \fi%
    \RightTagForm}%
  \xdef\@heading{%
    \LeftTagForm%
    \ifnum\Thm@nro=0
    \else\ifnum\Sec@nro=0 \theThm
	 \else
    		\ifnum\SubSec@nro=0 \theThm %%\theSec.\theThm
                \else\theSec.\theSubSec.\theThm
        	\fi
	 \fi
    \fi%
    \RightTagForm
}\@heading} %GRG
\def\Thm#1{\stepbyone{Thm}\Thm@{#1}}

\def\Sec@#1{\setcounter{SubSec}0\setcounter{Thm}0%
   \xdef\@currentlabel{Section \ifnum\Sec@nro=0\else\theSec\fi}
   \xdef\@currentcontentsentry{#1}
  \xdef\@heading{%
    \ifnum\Sec@nro=0\else\theSec\fi}\@heading}
\def\Sec#1{\stepbyone{Sec}\Sec@{#1}}

\def\SubSec@{\setcounter{Thm}0%
\xdef\@currentlabel{Section\ifnum\SubSec@nro=0\else \theSec.\theSubSec\fi}%
\xdef\@heading{\ifnum\SubSec@nro=0\else \theSec.\theSubSec\fi}\@heading}

\def\SubSec{\stepbyone{SubSec}\SubSec@}

\def\Item@{\xdef\@currentlabel{\LeftTagForm
    \ifnum\Item@nro=0 \else\romannumeral\theItem\fi\RightTagForm}%
  \@currentlabel}
\def\Item{\stepbyone{Item}\Item@}

%\def\proclaim#1#2#3{\setcounter{Item}0\smallskip\goodbreak
%   \thmskip\flushpar\Thm{#3}\label{#1}{\it #2}\nobreak\smallskip\nobreak\flushpar}
\def\cor#1#2{\proclaim{#1}{#2}{Corollary}}
\def\defn#1#2{\proclaim{#1}{#2}{Definition}}
\def\lemma#1#2{\proclaim{#1}{#2}{Lemma}}
\def\note#1#2{\proclaim{#1}{#2}{Note}}
\def\prop#1#2{\proclaim{#1}{#2}{Proposition}}
\def\thm#1#2{\proclaim{#1}{#2}{Theorem}}
\def\proof{\smallskip\flushpar{\smc Proof.}\quad}
\def\sketchproof{\smallskip\flushpar{\smc Sketch Proof.}\quad}
\def\temp#1{\smallskip\flushpar{\hbox{{\smc Temporary details:}} #1}{\hfil$\spadesuit$\linebreak}\flushpar}
\def\thmskip{\vskip10pt}

\def\item#1#2{\flushpar{\hbox{\hbox to1cm{\rm\Item}\label{#1}\hfil} #2\hfil}}
\def\Proofitem#1#2{\flushpar{\hbox{\refer{#1}} #2}\flushpar}

\def\LeftTagForm{}
\def\RightTagForm{}
\def\Tag@{\xdef\@currentlabel{\LeftTagForm%
    \ifnum\Thm@nro=0
    \else\ifnum\Sec@nro=0 \theThm
	 \else
    		\ifnum\SubSec@nro=0 \theSec.\theThm
                \else\theSec.\theSubSec.\theThm
        	\fi
	 \fi
    \fi%
    \RightTagForm}%
  \@currentlabel}
\def\Tag{\stepbyone{Thm}\Tag@}
 
%\catcode`\@=\active
%
%   END EDITING
%================================================================
 
%    ********************************
%    *   CROSS REFERENCING MACROS   *
%    ********************************
%
%  The user writes  \label{foo}  to define the following cross-references:
%     \ref{foo}     : value of most recently incremented referencable counter.
%       (Chapter, section, theorem, tag, figure, table and roster's item
%        counters are referencable, footnote counters are not.)
%     \pageref{foo} : page number at which \label{foo} command appeared.
%  where  foo  can be any string of characters not containing '\', '{' or '}'.
%
 
\def\thepage{\number\pageno}
 
\def\refer#1{\@ifundefined{r@#1}{{ ??}\global\@fwdreftrue\@warning
   {Reference `#1' on page \thepage \space
    undefined}}{\edef\@tempa{\@nameuse{r@#1}}\expandafter
    \@car\@tempa \@nil\null}}
 
\def\referpage#1{\@ifundefined{r@#1}{{ ??}\global\@fwdreftrue\@warning
   {Reference `#1' on page \thepage \space
    undefined}}{\edef\@tempa{\@nameuse{r@#1}}\expandafter
    \@cdr\@tempa\@nil\null}}
 
\newif\if@filesw \@fileswtrue
 
\def\label#1{\@bsphack\if@filesw {\let\thepage\relax
   \xdef\@gtempa{\write\@auxout{\string
      \newlabel{#1}{{\@currentlabel}{\thepage}}}}}\@gtempa
   \fi\@esphack}
 
\def\contentsentry#1{\@bsphack\if@filesw {\let\thepage\relax
   \xdef\@gtempa{\write\@auxout{\string
      \newcontentsentry{#1}{{\@currentlabel}{\thepage}}}}}\@gtempa
   \fi\@esphack}
 
 
% \rosterlabel is AmSTeX-specific
\def\rosterlabel#1{\@bsphack\xdef\@currentlabel{%
   \therosteritem{\number\rostercount@}}%
   \if@filesw {\let\thepage\relax
   \xdef\@gtempa{\write\@auxout{\string
      \newlabel{#1}{{\@currentlabel}{\thepage}}}}}\@gtempa
   \fi\@esphack}
 
\def\newlabel#1#2{\@ifundefined{r@#1}{}{\@warning{Label `#1' multiply
   defined}}\global\@namedef{r@#1}{#2}}
 
\def\@currentlabel{} % For \label commands that come before any environment
 
%     ****************
%     *   INDEXing   *
%     ****************
% This is quite primitive
%
\newif\if@indexsw
\newwrite\@idxout
 
\def\makeindex{\@indexswtrue\immediate\openout\@idxout=\jobname.idx
   \immediate\write\@idxout{\string\relax}}
 
\def\index#1{\@bsphack\if@indexsw {\let\thepage\relax
   \xdef\@gtempa{\write\@idxout{\string
      \indexentry{#1}{\thepage}}}}\@gtempa
   \fi\@esphack}
 
\def\indexentry#1#2{\noindent {#1}{\unskip\nobreak\hfil\penalty50
   \hskip2em\hbox{}\nobreak\hfil#2%
   \parfillskip=0pt \finalhyphendemerits=0 \par}}
 
%      **************************
%      *       CITATIONS        *
%      **************************
%      These are AmS-TeX specific
%
%  CONVENTION
%  \b@FOO : The name or number of the reference created by \citeto{FOO}
%     E.g., if \citeto{FOO} -> [17] , then \b@FOO -> 17.
%
\def\make@ref#1{\@ifundefined{b@#1}{{??}\global\@fwdreftrue\@warning
   {Citation `#1' on page \thepage \space
    undefined}}{\@nameuse{b@#1}}}
%
% FROM AMSTEX.TEX
%\newif\ifin@
%\def\in@#1#2{\def\in@@##1#1##2##3\in@@{\ifx\in@##2\in@false\else\in@true\fi}%
% \in@@#2#1\in@\in@@}
%
\def\citeto#1{\relaxnext@
 \def\nextiii@##1,##2\end@{\immediate\write\@auxout{\string\citation{##1}}%
   {\make@ref{##1}},##2}%
 \in@,{#1}\ifin@\def\next{\nextiii@#1\end@}\else
   \def\next{\immediate\write\@auxout{\string\citation{#1}}%
     {\make@ref{#1}}}\fi
     \next}
\def\noOf#1{\global\advance\c@num by1
   \if@filesw \immediate\write\@auxout
   {\string\bibcite{#1}{\the\c@num}}\fi\no\make@ref{#1}}
\def\keyOf#1#2{\if@filesw
   {\def\protect##1{\string ##1\space}\immediate
   \write\@auxout{\string\bibcite{#1}{#2}}}\fi
   \key{$\lbrack${\bf #2}$\rbrack$}}
 
\def\TAG{\tag"\Tag"}
% AmSTeXin pitaa joissakin komennoissaan voida nahda \tag suoraan
% joilloin komentoa \TAG ei voi kayttaa, vaan tulee kirjoittaa \tag"\Tag"
% Tassa pitaa kayttaa AmSTeXin \tagin literaalista optiota \tag"...",
% silla numerossa \Tag ovat sulut (...) mukana.
% Jos sulkujen muotoa halutaan muuttaa, ovat sulut maariteltyna nimilla
% \LeftTagForm (vasen kaarisulku) ja \RightTagForm (oikea kaarisulku).
% Siis: \redefine\LeftTagForm{...} (tarvittaessa \predefine ...).
% ==========================================================================
\let\@@end=\end
\let\@@supereject=\supereject
\def\supereject{\@@supereject}
\def\end{\if@fwdref
  \typeout{Undefined forward references/citations. Rerun.}\fi
  \@@end}
%
% PLAINin \bye
%\def\bye{\par\vfill\supereject\end}
%
% AMSTEXin \enddocument
%\outer\def\enddocument{\nobreak\sfcode`\.=3000 \vskip12\p@ minus6\p@
% \thekeywords@\thesubjclass@\nobreak\vskip12\p@ minus6\p@\addressnum@\z@
% \loop\ifnum\addressnum@<\addresscount@\advance\addressnum@\@ne
% \csname address\number\addressnum@\endcsname\repeat
% \vfill\supereject\end}
 
%      **************************
%      *     USEFUL HACKS       *
%      **************************
%
%  \@namedef{NAME}   : Expands to \def\NAME , except name can contain any
%         characters.
%  \@nameuse{NAME}   : Expands to \NAME .
%  \@ifnextchar X{YES}{NO}
%       : Expands to YES if next character is an 'X',
%         and to NO otherwise. (Uses temps a-c.)
%         NOTE: GOBBLES ANY SPACE FOLLOWING IT.
%  \@ifundefined{NAME}{YES}{NO}
%       : If \NAME is undefined then it executes YES,
%         otherwise it executes NO.  More precisely,
%         true if \NAME either undefined or = \relax.
%  \@car T1 T2 ... Tn\@nil == T1  (unexpanded)
%  \@cdr T1 T2 ... Tn\@nil == T2 ... Tn     (unexpanded)
%  \typeout{message} : produces a warning message on the terminal
%  \@warning{message}: prints 'Warning: message.'
%
\newwrite\@unused
\def\typeout#1{{\let\protect\string\immediate\write\@unused{#1}}}
\def\@warning#1{\typeout{Warning: #1.}}
 
\def\@namedef#1{\expandafter\def\csname #1\endcsname}
\def\@nameuse#1{\csname #1\endcsname}
 
\def\@car#1#2\@nil{#1}
\def\@cdr#1#2\@nil{#2}
 
\long\def\@ifundefined#1#2#3{\expandafter\ifx\csname
  #1\endcsname\relax#2\else#3\fi}
 
\def\@ifnextchar#1#2#3{\let\@tempe #1\def\@tempa{#2}\def\@tempb{#3}\futurelet
    \@tempc\@ifnch}
\def\@ifnch{\ifx \@tempc \@sptoken \let\@tempd\@xifnch
      \else \ifx \@tempc \@tempe\let\@tempd\@tempa\else\let\@tempd\@tempb\fi
      \fi \@tempd}
 
\def\?{\let\@sptoken= } \?  % this makes \@sptoken a space token
 
\def\?{\@xifnch} \expandafter\def\? {\futurelet\@tempc\@ifnch}
 
% SPACE HACKS
% \@bsphack ... \@esphack
%     used by macros such as \index and \label
%     that want to be invisible -- i.e.,
%     not leave any extra space when used in the middle of text.  Such
%     a macro should begin with \@bsphack and end with \@esphack
%     The macro in question should not create any text, nor change the
%     mode.
%
\newdimen\@savsk
\newcount\@savsf
 
\def\@bsphack{\@savsk\lastskip
    \ifhmode\@savsf\spacefactor\fi}
 
\def\@esphack{\relax\ifhmode\spacefactor\@savsf
     {}\ifdim \@savsk >\z@ \ignorespaces\fi\fi}
 
%     **************************
%     *    FILE HANDLING       *
%     **************************
%
%    \Input{foo} : If file foo exists, then \input's it,
%                  otherwise types a warning message.
\def\Input#1{\openin1 #1 \ifeof1 \typeout{No file #1.}\closein1
    \else\closein1 \relax\input #1 \fi}
 
%      **************************
%      *     BIBLIOGRAPHY       *
%      **************************
%
\newcount\c@num \c@num=0
 
\def\bibcite#1#2{\@ifundefined{r@#1}{}{\@warning{Referencelabel `#1' multiply
   defined}}\global\@namedef{b@#1}{#2}}
 
\def\@gobble#1{}
\let\citation\@gobble
 
%      **************************
%      *      INSERTIONS        *
%      **************************
%
% AMSTEX.TEXin \ins@ (\midspace...) MUUTETTU
%
% Jos \ins@:n \caption ulottuu kahdelle riville
% tulisi \captionissa mahd. esiintyva \Fig sovellettua
% kahdesti ja \Fig-numero kasvaisi kahdella
%
\def\CorrectCounter{}
%\newif\ifmid@
%\def\topspace{\mid@false\ins@}
%\def\midspace{\mid@true\ins@}
\def\ins@#1{\relaxnext@
 \smallcaptionwidth@\captionwidth@\gdef\thespace@{#1}%
 \def\next@{\ifx\next\space@\def\next. {\futurelet\next\nextii@}\else
  \def\next.{\futurelet\next\nextii@}\fi\next.}%
 \def\nextii@{\ifx\next\caption\def\next\caption{\futurelet\next\nextiii@}%
  \else\let\next\nextiv@\fi\next}%
 \def\nextiv@{\vnonvmode@
  {\ifmid@\let\next\midinsert\else\let\next\topinsert\fi
  \next\vbox to\thespace@{}\endinsert}
  {\ifmid@\nonvmodeerr@\midspace\else\nonvmodeerr@\topspace\fi}}%
 \def\nextiii@{\ifx\next\captionwidth\let\next\nextv@
  \else\let\next\nextvi@\fi\next}%
 \def\nextv@\captionwidth##1##2{\smallcaptionwidth@##1\relax\nextvi@{##2}}%
 \def\nextvi@##1{\def\thecaption@{##1}%
  \def\next@{\ifx\next\space@\def\next. {\futurelet\next\nextvii@}\else
   \def\next.{\futurelet\next\nextvii@}\fi\next.}%
  \futurelet\next\next@}%
 \def\nextvii@{\vnonvmode@
  {\ifmid@\let\next\midinsert\else
  \let\next\topinsert\fi\next\vbox to\thespace@{}\nobreak\smallskip
  \setbox\z@\hbox{\noindent\ignorespaces\thecaption@\unskip}%
  \ifdim\wd\z@>\smallcaptionwidth@\centerline{\vbox{\hsize\smallcaptionwidth@
  \noindent\ignorespaces\CorrectCounter\thecaption@
  \gdef\CorrectCounter{}\unskip}}%
  \else\centerline{\box\z@}\fi\endinsert}
  {\ifmid@\nonvmodeerr@\midspace
  \else\nonvmodeerr@\topspace\fi}}%
 \futurelet\next\next@}
% END OF \ins@ MODIFICATION
%
%
%      **************************
%      *     INITIALIZATION     *
%      **************************
\Input{\jobname.aux}
\immediate\openout\@auxout=\jobname.aux
\immediate\write\@auxout{\string\relax}
\catcode`\@=\active

